Dual Averaging is Surprisingly Effective for Deep Learning Optimization

First-order stochastic optimization methods are currently the most widely used class of methods for training deep neural networks. However, the choice of the optimizer has become an ad-hoc rule that can significantly affect the performance. For instance, SGD with momentum (SGD+M) is typically used in computer vision (CV) and Adam is used for training transformer models for Natural Language Processing (NLP). Using the wrong method can lead to significant performance degradation. Inspired by the dual averaging algorithm, we propose Modernized Dual Averaging (MDA), an optimizer that is able to perform as well as SGD+M in CV and as Adam in NLP. Our method is not adaptive and is significantly simpler than Adam. We show that MDA induces a decaying uncentered $L_2$-regularization compared to vanilla SGD+M and hypothesize that this may explain why it works on NLP problems where SGD+M fails.

==> completemdaproof.tex <==
% TeXShop support
% !TEX root = main.tex


\iffalse

\begin{theorem}\label{thm:mda}
  Let $f$ be a Lipschitz-smooth function. Let \autoref{ass:sto_grad} and \autoref{ass:bounddomain} for \eqref{eq:prob} hold. Let $z_1,\dots,z_T$ and $x_1,\dots,x_T$ be the points returned by MDA and set $\lambda_k=\Lambda \sqrt{k+1}$, $\beta_k=\sqrt{k+1}$ and $c_k=c$ where $\Lambda =1/\sqrt{T}$ and $c\in (0,1].$ Then, we have:
  \begin{equation}\label{eq:da_rate}
\begin{split}
        &\frac{1}{T}\sum_{k=0}^T\|\nabla f(x_k)\|_2^2+\frac{1}{T}\sum_{k=0}^T\|\nabla f(z_k)\|_2^2\\
        &\leq \frac{4(f(x_{0})-\mathbb{E}[f(z_{T+1})])}{\sqrt{T}}+4\left(\frac{1}{c}-1\right)\frac{(L+1)f(x_{0})-(L+\alpha_T)\mathbb{E}[f(x_{T})] }{T} \\
    &-\left(\frac{1}{c}-1\right)\frac{1}{\sqrt{T}}\sum_{k=0}^T\frac{f(x_{k})}{ (k+2)^{3/2}\sqrt{k+3}}\\
    %
    %
    %
        &+  \left(\frac{4L}{\sqrt{T}} +\frac{2\log(T+1)}{T}\right)\sigma^2+ \left( \frac{2L\log(T)}{T}+\frac{4\log(T)}{\sqrt{T}}  +\frac{\zeta(2)}{\sqrt{T} }\right) R^2\\
       % &+(L+\alpha_k) \alpha_kR^2+\frac{\alpha_kR^2}{\eta_k} \\
    &+  \left[\left(L+\sqrt{T}\right)\left(\frac{1}{c}-1\right)^2+L\left(\frac{1}{c}-1\right)-\frac{\sqrt{T}}{  c^2}\right]\frac{2L}{T}\sum_{k=0}^T\|x_k-x_{k-1}\|_2^2\\
    &+  \left[\left(L+\sqrt{T}\right)\left(\frac{1}{c}-1\right)^2+ \left(\frac{1}{c}-1\right)\left(L+1+\frac{\sqrt{T}}{2 c} \right)-\frac{\sqrt{T}}{ c^2}  \right]\frac{1}{T}\sum_{k=0}^T\frac{\|x_k-x_{k-1}\|_2^2}{k+1}\\
    &+\left(\frac{1}{c}-1\right) \frac{1}{2 c\sqrt{T}}\sum_{k=0}^T\frac{\|x_k-x_{k-1}\|_2^2}{(k+1)^2}.
 \end{split}
\end{equation}
\end{theorem}

\fi




























\section{Convergence analysis of MDA}\label{sec:mda_proof}

This section is dedicated to the convergence proof of MDA. To obtain the rate in \autoref{thm:mda}, we use \autoref{prop:mdda} and \autoref{thm:sgd_rate}. We start by introducing some notations. 

\subsection{Notations and useful inequalities}

At a fixed step step $k$, we remind that the function $h^{(k)}\colon \mathbb{R}^n\rightarrow \mathbb{R}$ is defined as
\begin{align}\label{eq:hk}
      h^{(k)}(x)&=f(x)+\frac{\alpha_k}{2}\|x-x_0\|^2.
 \end{align}
 We now introduce the following notions induced by $ h^{(k)}.$ $\Gamma_{k+1}$ is the Lyapunov function with respect to $h^{(k)}$ and is defined as 
\begin{align}\label{eq:lyap_def}
    \Gamma_{k+1}:=\frac{1}{\eta_{k}^2}h^{(k)}(z_{k+1}) +\frac{L_{h^{(k)}}}{\eta_k}\left(\frac{1}{c_k}-1\right)h^{(k)}(x_k)+\frac{1}{2}\frac{L_{h^{(k)}}}{\eta_k^2 c_{k+1}^2}\|x_{k+1}-x_k\|_2^2,
\end{align}
 $\nabla h^{(k)}(x_k,\xi_k)$ is the stochastic gradient of $h^{(k)}$ and is equal to
 \begin{align}\label{eq:nablah}
     \nabla h^{(k)}(x_k,\xi_k):=\nabla f(x_k,\xi_k)+\alpha_k(x_k-x_0),
 \end{align}
 
and $L_{h^{(k)}}$ is the smoothness constant of $h^{(k)}$,
 \begin{align}\label{eq:Lhk}
     L_{h^{(k)}}:=L+\alpha_k.
 \end{align}
 We remind that with our parameters choices \eqref{eq:params_noncvx}, we have:
\begin{align}\label{eq:remind_params}
    \alpha_k = \frac{\sqrt{k+2}-\sqrt{k+1}}{\Lambda \sqrt{k+2}},  \quad \quad \eta_k=\Lambda \quad \text{ and } \quad c_k=c \qquad \text{where } \Lambda >0\text{ and }c \in (0,1).
\end{align}
Therefore, $ \alpha_k $ is a non-increasing sequence and as a consequence, \begin{align}\label{eq:decrease_alpha}
\alpha_{k+1}-\alpha_k\leq 0.
\end{align}
It can further be shown that 
\begin{align}\label{eq:alphakk1diff}
    \alpha_{k}(\alpha_{k+1}-\alpha_k)\leq 0,
\end{align}
and
\begin{align}\label{eq:alphakk1diff1}
    \alpha_{k+1}(\alpha_{k+1}-\alpha_k)\leq 0.
\end{align}
Moreover, by using the inequality $\sqrt{k+2}-\sqrt{k+1} \leq (2\sqrt{k+1})^{-1}$, we have:
\begin{align}
    \alpha_k \leq \frac{1}{2\Lambda(k+1)}.
\end{align}
We will encounter the quantity $\alpha_{k+1}-\alpha_k$ in the proof and would like to upper bound it. We first start by upper bounding $\alpha_{k+1}-\alpha_k:$
\begin{align}
    \alpha_{k+1}-\alpha_k&=  \frac{\sqrt{k+3}-\sqrt{k+2}}{\Lambda\sqrt{k+3}}- \frac{\sqrt{k+2}-\sqrt{k+1}}{ \Lambda\sqrt{k+2}} \nonumber\\
    &\leq \frac{1}{2\Lambda\sqrt{(k+3)(k+2)}}- \frac{1}{2 \Lambda(k+2)}\label{eq:23}\\
    &= \frac{1}{2\Lambda \sqrt{k+2}}\frac{\sqrt{k+2}-\sqrt{k+3}}{\sqrt{(k+2)(k+3)}} \nonumber\\
    &\leq -\frac{1}{4\Lambda (k+2)^{3/2}\sqrt{k+3}},\label{eq:24}
\end{align}
where we used the inequalities for any $x>1,$ $\sqrt{x-1}-\sqrt{x}\leq -(2\sqrt{x})^{-1}$ in \eqref{eq:23} and \eqref{eq:24} and for any $x>0,$ $\sqrt{x+1}-\sqrt{x}\leq (2\sqrt{x})^{-1}$ in \eqref{eq:23}.

\subsection{Proof of \autoref{thm:mda}}

\paragraph{Adapting the proof of non-convex SPA.} We start off by using the inequality satisfied by non-convex SPA (\autoref{thm:sgd_rate}). By applying it to $ h^{(k)}$, we obtain:
\begin{equation}\label{eq:daexpupdsmooth}
\begin{split}
        \frac{1}{2\eta_k}\|\nabla h^{(k)}(x_k)\|_2^2+\frac{1}{2\eta_k}\|\nabla h^{(k)}(z_k)\|_2^2 &\leq \Gamma_k-\mathbb{E}_{k}[\Gamma_{k+1}]+  L_{h^{(k)}}  \mathbb{E}_{k}[\|\nabla h^{(k)}(x_k,\xi_k)\|_2^2]\\
    &+\frac{1}{2}\left[\frac{1}{\eta_k^2}\left(\frac{1}{c_k}-1+\eta_kL_{h^{(k)}}\right)\left(\frac{1}{c_k}-1\right)\right.\\
    &\left.+\frac{1}{\eta_k}L_{h^{(k)}}\left(\frac{1}{c_k}-1\right)^2-\frac{1}{\eta_{k-1}^2c_k^2}\right]L_{h^{(k)}}\|x_k-x_{k-1}\|_2^2.
\end{split}
\end{equation}

By using \eqref{eq:nablah} and the inequality $\|a+b\|_2^2 \leq 2\|a\|_2^2 +2\|b\|_2^2$ for $a,b\in\mathbb{R}^n$ in \eqref{eq:daexpupdsmooth}, we obtain:
 \begin{equation}\label{eq:daexpupdsmoothineq}
\begin{split}
        \frac{1}{4\eta_k}\|\nabla f(x_k)\|_2^2+\frac{1}{4\eta_k}\|\nabla f(z_k)\|_2^2 &\leq \Gamma_k-\mathbb{E}_{k}[\Gamma_{k+1}]+  L_{h^{(k)}}  \mathbb{E}_{k}[\|\nabla f(x_k,\xi_k)\|_2^2]\\
        &+L_{h^{(k)}} \alpha_k\|x_k-x_0\|_2^2+\frac{\alpha_k}{2\eta_k}\left(\|x_k-x_0\|_2^2+\|z_k-x_0\|_2^2\right)\\
    &+\frac{1}{2}\left[\frac{1}{\eta_k^2}\left(\frac{1}{c_k}-1+\eta_kL_{h^{(k)}}\right)\left(\frac{1}{c_k}-1\right)\right.\\
    &\left.+\frac{1}{\eta_k}L_{h^{(k)}}\left(\frac{1}{c_k}-1\right)^2-\frac{1}{\eta_{k-1}^2c_k^2}\right]L_{h^{(k)}}\|x_k-x_{k-1}\|_2^2,
\end{split}
\end{equation}
Now, by using the definition \eqref{eq:Lhk} of $ L_{h^{(k)}}$, the choice of parameters \eqref{eq:remind_params}, the boundedness assumption (\autoref{ass:bounddomain}) and the properties on the stochastic oracle (\autoref{ass:sto_grad}), \eqref{eq:daexpupdsmoothineq} becomes: 
 \begin{equation}\label{eq:finalbeforelyap}
\begin{split}
        &\frac{1}{4\Lambda}\|\nabla f(x_k)\|_2^2+\frac{1}{4\Lambda}\|\nabla f(z_k)\|_2^2\\
        \leq& \Gamma_k-\mathbb{E}_{k}[\Gamma_{k+1}]+  \left(L +\frac{1}{2\Lambda(k+1)}\right)\sigma^2+ \frac{R^2}{2\Lambda(k+1)}\left(\frac{1}{\Lambda}+L+\frac{1}{2\Lambda(k+1)} \right)\\
       % &+(L+\alpha_k) \alpha_kR^2+\frac{\alpha_kR^2}{\eta_k} \\
    +&\left(\frac{L}{2}+ \frac{1}{4\Lambda(k+1)}\right)\left[\frac{1}{\Lambda^2}\left(\frac{1}{c}-1+\Lambda\left(L+\frac{1}{2\Lambda(k+1)}\right)\right)\left(\frac{1}{c}-1\right)\right.\\
    &\left.+\frac{1}{\Lambda}\left(L+\frac{1}{2\Lambda(k+1)}\right)\left(\frac{1}{c}-1\right)^2-\frac{1}{\Lambda^2c^2}\right]\|x_k-x_{k-1}\|_2^2.
\end{split}
\end{equation}

The rest of the proof is dedicated to bouding the difference of Lyapunov functions in \eqref{eq:finalbeforelyap}. 

 \paragraph{Bound on the difference of Lyapunov functions.}  By using \eqref{eq:lyap_def}, the difference of Lyapunov functions is:
\begin{align}
    \Gamma_k-\mathbb{E}_{k}[\Gamma_{k+1}]&=\frac{1}{\eta_{k-1}^2}h^{(k)}(z_{k})-\frac{1}{\eta_{k}^2}\mathbb{E}_{k}[h^{(k)}(z_{k+1})]\label{eq:28}\\
    &+\frac{L_{h^{(k)}}}{\eta_{k-1}}\left(\frac{1}{c_{k-1}}-1\right)h^{(k)}(x_{k-1})-\frac{L_{h^{(k)}}}{\eta_k}\left(\frac{1}{c_k}-1\right)h^{(k)}(x_k)\label{eq:29}\\
    &+\frac{1}{2}\frac{L_{h^{(k)}}}{\eta_{k-1}^2 c_{k}^2}\|x_{k}-x_{k-1}\|_2^2-\frac{1}{2}\frac{L_{h^{(k)}}}{\eta_k^2 c_{k+1}^2}\|x_{k+1}-x_k\|_2^2.\label{eq:30}
\end{align}
We now expand each term in the equality above. We start off by looking at \eqref{eq:28}. By using the definition of $h^{(k)}$, this latter can be rewritten as: 
\begin{equation}
    \begin{split}\label{eq:new_28}
        &\frac{1}{\eta_{k-1}^2}h^{(k)}(z_{k})-\frac{1}{\eta_{k}^2}\mathbb{E}_{k}[h^{(k)}(z_{k+1})]\\
        =&\frac{1}{\Lambda^2}(f(z_{k})-f(z_{k+1}))+\frac{\alpha_k\|z_k-x_0\|_2^2-\alpha_{k+1}\|z_{k+1}-x_0\|_2^2}{\Lambda^2}+\frac{\alpha_{k+1}-\alpha_{k}}{\Lambda^2}\|z_{k+1}-x_0\|_2^2\\
        \leq& \frac{1}{\Lambda^2}(f(z_{k})-f(z_{k+1}))+\frac{\alpha_k\|z_k-x_0\|_2^2-\alpha_{k+1}\|z_{k+1}-x_0\|_2^2}{\Lambda^2},
    \end{split}
\end{equation}
where we used \eqref{eq:decrease_alpha}. We now turn to \eqref{eq:29} and obtain: 
\begin{equation}
    \begin{split}\label{eq:29_new}
    &\frac{L_{h^{(k)}}}{\eta_{k-1}}\left(\frac{1}{c_{k-1}}-1\right)h^{(k)}(x_{k-1})-\frac{L_{h^{(k)}}}{\eta_k}\left(\frac{1}{c_k}-1\right)h^{(k)}(x_k)\\
    =&\frac{L}{\Lambda}\left(\frac{1}{c}-1\right)\left[f(x_{k-1})-f(x_{k}) +\frac{\alpha_k}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}}{2}\|x_k-x_0\|_2^2  \right] \\
    +&\frac{\alpha_k}{\Lambda}\left(\frac{1}{c}-1\right)\left[f(x_{k-1})-f(x_{k}) +\frac{\alpha_k}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}}{2}\|x_k-x_0\|_2^2  \right]  \\
    +&\frac{L+\alpha_k}{\Lambda}\left(\frac{1}{c}-1\right)(\alpha_{k+1}-\alpha_{k})\|x_k-x_0\|_2^2.
    \end{split}
\end{equation}
By using \eqref{eq:decrease_alpha} and \eqref{eq:alphakk1diff}, the last term in \eqref{eq:29_new} can be bounded as: 
\begin{align}\label{eq:dec29}
    \frac{L+\alpha_k}{\eta}\left(\frac{1}{c}-1\right)(\alpha_{k+1}-\alpha_{k})\|x_k-x_0\|_2^2&\leq 0.
\end{align}
The second term in \eqref{eq:29_new} can be rewritten as
\begin{equation}
    \begin{split}\label{eq:29_newnew}
        &\frac{\alpha_k}{\Lambda}\left(\frac{1}{c}-1\right)\left[f(x_{k-1})-f(x_{k}) +\frac{\alpha_k}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}}{2}\|x_k-x_0\|_2^2  \right]\\
        =&\frac{1}{\Lambda}\left(\frac{1}{c}-1\right)\left[\alpha_kf(x_{k-1})-\alpha_{k+1}f(x_{k}) +\frac{\alpha_k^2}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}^2}{2}\|x_k-x_0\|_2^2  \right]\\
    +&\frac{1}{\Lambda}\left(\frac{1}{c}-1\right)(\alpha_{k+1}-\alpha_k) f(x_{k}) +\frac{1}{\Lambda}\left(\frac{1}{c}-1\right)(\alpha_{k+1}-\alpha_k)  \frac{\alpha_{k+1}}{2}\|x_{k+1}-x_0\|_2^2.
    \end{split}
\end{equation}
By using \eqref{eq:alphakk1diff1} and \eqref{eq:24}, \eqref{eq:29_newnew} becomes
\begin{equation}
    \begin{split}\label{eq:29_newnewnew}
        &\frac{\alpha_k}{\Lambda}\left(\frac{1}{c}-1\right)\left[f(x_{k-1})-f(x_{k}) +\frac{\alpha_k}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}}{2}\|x_k-x_0\|_2^2  \right]\\
        \leq&\frac{1}{\Lambda}\left(\frac{1}{c}-1\right)\left[\alpha_kf(x_{k-1})-\alpha_{k+1}f(x_{k}) +\frac{\alpha_k^2}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}^2}{2}\|x_k-x_0\|_2^2  \right]\\
    -&\frac{1}{\Lambda}\left(\frac{1}{c}-1\right)\frac{f(x_{k})}{4\Lambda (k+2)^{3/2}\sqrt{k+3}} .
    \end{split}
\end{equation}


Finally, we deal with \eqref{eq:30}.
\begin{equation}\label{eq:new_30}
    \begin{split}
        &\frac{1}{2}\frac{L_{h^{(k)}}}{\eta_{k-1}^2 c_{k}^2}\|x_{k}-x_{k-1}\|_2^2-\frac{1}{2}\frac{L_{h^{(k)}}}{\eta_k^2 c_{k+1}^2}\|x_{k+1}-x_k\|_2^2\\
        =&\frac{1}{2}\frac{L}{\Lambda^2  c^2}(\|x_{k}-x_{k-1}\|_2^2-\|x_{k+1}-x_k\|_2^2)+\frac{1}{2\Lambda^2 c^2}(\alpha_k\|x_{k}-x_{k-1}\|_2^2-\alpha_{k+1}\|x_{k+1}-x_k\|_2^2)\\
    +&\frac{\alpha_{k+1}-\alpha_k}{2\Lambda^2 c^2}\|x_{k+1}-x_k\|_2^2.
    \end{split}
\end{equation}
By using \eqref{eq:decrease_alpha}, the last term in \eqref{eq:new_30} is upper bounded
\begin{align}\label{eq:dec30}
    \frac{\alpha_{k+1}-\alpha_k}{2\Lambda^2 c^2}\|x_{k+1}-x_k\|_2^2\leq 0.
\end{align}


Now, by assembling \eqref{eq:new_28}, \eqref{eq:29_new}, \eqref{eq:new_30}, \eqref{eq:29_newnewnew}, \eqref{eq:new_30} and \eqref{eq:dec30}, we have
\begin{equation}
    \begin{split}\label{eq:final_lyap_diff}
        \Gamma_k-\mathbb{E}_{k}[\Gamma_{k+1}]
        &\leq \frac{1}{\Lambda^2}(f(z_{k})-f(z_{k+1}))+\frac{\alpha_k\|z_k-x_0\|_2^2-\alpha_{k+1}\|z_{k+1}-x_0\|_2^2}{\Lambda^2}\\
    &+\frac{L}{\Lambda}\left(\frac{1}{c}-1\right)\left[f(x_{k-1})-f(x_{k}) +\frac{\alpha_k}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}}{2}\|x_k-x_0\|_2^2  \right] \\
&+\frac{1}{\Lambda}\left(\frac{1}{c}-1\right)\left[\alpha_kf(x_{k-1})-\alpha_{k+1}f(x_{k}) +\frac{\alpha_k^2}{2}\|x_{k-1}-x_0\|_2^2\right.\\
&\left.-\frac{\alpha_{k+1}^2}{2}\|x_k-x_0\|_2^2  \right]\\
    &-\frac{1}{\Lambda}\left(\frac{1}{c}-1\right)\frac{f(x_{k})}{4\Lambda (k+2)^{3/2}\sqrt{k+3}}\\
    &+\frac{1}{2}\frac{L}{\Lambda^2  c^2}(\|x_{k}-x_{k-1}\|_2^2-\|x_{k+1}-x_k\|_2^2)\\
    &+\frac{1}{2\Lambda^2 c^2}(\alpha_k\|x_{k}-x_{k-1}\|_2^2-\alpha_{k+1}\|x_{k+1}-x_k\|_2^2).
    \end{split}
\end{equation}


























 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\

\iffalse


As $\eta_k$ and $c_k$ are constant, we have
\begin{align}
    \Gamma_k-\mathbb{E}_{k}[\Gamma_{k+1}]&=\frac{1}{\eta^2}(f(z_{k})-f(z_{k+1})) +\frac{\alpha_k\|z_k-x_0\|_2^2-\alpha_{k+1}\|z_{k+1}-x_0\|_2^2}{\eta^2}\\
    &+\frac{\alpha_{k+1}-\alpha_{k}}{\eta^2}\|z_{k+1}-x_0\|_2^2\label{eq:28}\\
    &+\frac{L}{\eta}\left(\frac{1}{c}-1\right)\left[f(x_{k-1})-f(x_{k}) +\frac{\alpha_k}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}}{2}\|x_k-x_0\|_2^2  \right] \\
    &+\frac{\alpha_k}{\eta}\left(\frac{1}{c}-1\right)\left[f(x_{k-1})-f(x_{k}) +\frac{\alpha_k}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}}{2}\|x_k-x_0\|_2^2  \right]\label{eq:30} \\
    &+\frac{L+\alpha_k}{\eta}\left(\frac{1}{c}-1\right)(\alpha_{k+1}-\alpha_{k})\|x_k-x_0\|_2^2\\
    &+\frac{1}{2}\frac{L}{\eta^2  c^2}(\|x_{k}-x_{k-1}\|_2^2-\|x_{k+1}-x_k\|_2^2)\\
    &+\frac{1}{2\eta^2 c^2}(\alpha_k\|x_{k}-x_{k-1}\|_2^2-\alpha_{k+1}\|x_{k+1}-x_k\|_2^2)\\
    &+\frac{\alpha_{k+1}-\alpha_k}{2\eta^2 c^2}\|x_{k+1}-x_k\|_2^2.\label{eq:34}
\end{align}
%+\alpha_k
We remark that the terms in \eqref{eq:28} and \eqref{eq:34} are non-positive as $\alpha_k$ is a non-increasing sequence. Remark that all the terms above are telescopic except \eqref{eq:30}. We now rewrite \eqref{eq:30}. 

\begin{align}
    \eqref{eq:30}&= \frac{1}{\eta}\left(\frac{1}{c}-1\right)\left[\alpha_kf(x_{k-1})-\alpha_{k+1}f(x_{k}) +\frac{\alpha_k^2}{2}\|x_{k-1}-x_0\|_2^2-\frac{\alpha_{k+1}^2}{2}\|x_k-x_0\|_2^2  \right]\\
    &+\frac{1}{\eta}\left(\frac{1}{c}-1\right)(\alpha_{k+1}-\alpha_k) f(x_{k}) \\
    &+\frac{1}{\eta}\left(\frac{1}{c}-1\right)(\alpha_{k+1}-\alpha_k)  \frac{\alpha_{k+1}}{2}\|x_{k+1}-x_0\|_2^2.\label{eq:37}
\end{align}
Remark that \eqref{eq:37} is non-positive. Therefore, by summing  $\Gamma_k-\mathbb{E}_{k}[\Gamma_{k+1}]$ for $k=0,\dots,T$, we obtain
\begin{align}
    \Gamma_0-\mathbb{E}[\Gamma_{T+1}]&\leq\frac{1}{\eta^2}(f(z_{0})-f(z_{T+1})) +\frac{\alpha_0\|z_0-x_0\|_2^2}{\eta^2}\\
    &+\frac{L}{\eta}\left(\frac{1}{c}-1\right)\left[f(x_{0})-\mathbb{E}[f(x_{T+1})]   \right] \\
    &+\frac{1}{\eta}\left(\frac{1}{c}-1\right)\left[\alpha_0f(x_{0})-\alpha_{T+1}\mathbb{E}[f(x_{T})]  \right]\\
    &+\frac{1}{\eta}\left(\frac{1}{c}-1\right)\sum_{k=0}^T(\alpha_{k+1}-\alpha_k) f(x_{k})  \\
     &+\frac{1}{2\eta^2 c^2}\sum_{k=0}^T(\alpha_{k+1}-\alpha_k)\|x_{k+1}-x_k\|_2^2.
\end{align} 
 
\paragraph{Term in $\|x_k-x_{k-1}\|_2^2$} We develop the coefficient in front of $\|x_k-x_{k-1}\|_2^2$. We have

\begin{align}
&\left[\frac{1}{\eta_k^2}\left(\frac{1}{c_k}-1+\eta_kL_{h^{(k)}}\right)\left(\frac{1}{c_k}-1\right)+ \frac{1}{\eta_k}L_{h^{(k)}}\left(\frac{1}{c_k}-1\right)^2-\frac{1}{\eta_{k-1}^2c_k^2}\right]L_{h^{(k)}}\nonumber\\
=&\left[\frac{1}{\eta^2}\left(\frac{1}{c}-1+\eta L\right)\left(\frac{1}{c}-1\right)+ \frac{L}{\eta} \left(\frac{1}{c}-1\right)^2-\frac{1}{\eta^2c^2} + \frac{\alpha_k}{c\eta}\left(\frac{1}{c}-1\right) \right](L+\alpha_k).
\end{align}
\fi 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
 \paragraph{Finalizing the convergence bound.} By summing \eqref{eq:finalbeforelyap} for $k=0,\dots,T$ and plugging the bound \eqref{eq:final_lyap_diff} on the difference of Lyapunov functions, we obtain: 
 
  \begin{equation}\label{eq:finalalmost}
\begin{split}
        &\frac{1}{4T}\sum_{k=0}^T\|\nabla f(x_k)\|_2^2+\frac{1}{4T}\sum_{k=0}^T\|\nabla f(z_k)\|_2^2\\
        &\leq \frac{f(z_{0})-f(z_{T+1})}{\Lambda T}+\frac{\alpha_0\|z_0-x_0\|_2^2}{\Lambda T}+\left(\frac{1}{c}-1\right)\frac{(L+\alpha_0)f(x_{0})-(L+\alpha_T)f(x_{T}) }{T} \\
    &-\left(\frac{1}{c}-1\right)\frac{1}{4\Lambda T}\sum_{k=0}^T\frac{f(x_{k})}{ (k+2)^{3/2}\sqrt{k+3}}+\frac{1}{2}\frac{L+\alpha_0}{\Lambda c^2}(\|x_{0}-x_{-1}\|_2^2)\\
    %
    %
    %
        &+  \left(L\Lambda +\frac{1}{2T}\sum_{k=0}^T\frac{1}{k+1}\right)\sigma^2+ \left(\left(\frac{1}{\Lambda}+L \right)\frac{1}{2T} \sum_{k=0}^T\frac{1}{k+1}+\frac{1}{4\Lambda T }\sum_{k=0}^T\frac{1}{(k+1)^2}\right) R^2\\
       % &+(L+\alpha_k) \alpha_kR^2+\frac{\alpha_kR^2}{\eta_k} \\
    &+  \left[\left(L+\frac{1}{\Lambda}\right)\left(\frac{1}{c}-1\right)^2+L\left(\frac{1}{c}-1\right)-\frac{1}{\Lambda c^2}\right]\frac{L}{2T}\sum_{k=0}^T\|x_k-x_{k-1}\|_2^2\\
    &+  \left[\left(L+\frac{1}{\Lambda}\right)\left(\frac{1}{c}-1\right)^2+ \left(\frac{1}{c}-1\right)\left(L+1+\frac{1}{2\Lambda c} \right)-\frac{1}{\Lambda c^2}  \right]\frac{1}{4T}\sum_{k=0}^T\frac{\|x_k-x_{k-1}\|_2^2}{k+1}\\
    &+\left(\frac{1}{c}-1\right) \frac{1}{8\Lambda cT}\sum_{k=0}^T\frac{\|x_k-x_{k-1}\|_2^2}{(k+1)^2}.
    %\left(\frac{L\Lambda}{2}+ \frac{1}{4\Lambda(k+1)}\right)\left[\frac{1}{\Lambda^2}\left(\frac{1}{c}-1+\Lambda\left(L+\frac{1}{2\Lambda(k+1)}\right)\right)\left(\frac{1}{c}-1\right)\right.\\
  %  &\left.+\frac{1}{\Lambda}\left(L+\frac{1}{2\Lambda(k+1)}\right)\left(\frac{1}{c}-1\right)^2-\frac{1}{\Lambda^2c^2}\right]\|x_k-x_{k-1}\|_2^2
\end{split}
\end{equation}

By using the inequality $\sum_{k=0}^T \frac{1}{k+1}\leq \log(T+1)$ and setting $z_0=x_0$, $x_{-1}=x_0$ and $\Lambda=1/\sqrt{T}$, we obtain the aimed result.
 
 
 
 
 
 
 
 
 
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
 \iffalse
 
  \begin{equation}\label{eq:final1}
\begin{split}
        &\frac{1}{4T}\sum_{k=0}^T(\|\nabla f(x_k)\|_2^2+\|\nabla f(z_k)\|_2^2)\\
        &\leq \frac{1}{\eta T}(f(z_{0})-f(z_{T+1})) +\frac{\alpha_0\|z_0-x_0\|_2^2}{\eta T}\\
    &+\frac{L}{T}\left(\frac{1}{c}-1\right)\left[f(x_{0})-\mathbb{E}[f(x_{T+1})]   \right] \\
    &+\frac{1}{T}\left(\frac{1}{c}-1\right)\left[\alpha_0f(x_{0})-\alpha_{T+1}\mathbb{E}[f(x_{T})]  \right]\\
    &+\frac{1}{T}\left(\frac{1}{c}-1\right)\sum_{k=0}^T(\alpha_{k+1}-\alpha_k) f(x_{k})  \\
     %&+\frac{1}{2c^2\eta T }\sum_{k=0}^T(\alpha_{k+1}-\alpha_k)\|x_{k+1}-x_k\|_2^2.\\ 
     &+\left(L+\frac{1}{\eta T}\sum_{k=0}^T\frac{1}{k+1}\right)\eta\sigma^2+\left(L+\frac{1}{\eta T}\sum_{k=0}^T\frac{1}{k+1}\right)\eta R^2+\frac{R^2}{\eta T}\sum_{k=0}^T\frac{1}{k+1}\\
    &+\frac{L}{\eta T}\left[\frac{1}{\eta}\left(\frac{1}{c}-1+\eta L\right)\left(\frac{1}{c}-1\right)+ L \left(\frac{1}{c}-1\right)^2-\frac{1}{\eta c^2} \right] \sum_{k=0}^T\|x_k-x_{k-1}\|_2^2\\
    &+\frac{1}{\eta T}\left[\frac{1}{\eta}\left(\frac{1}{c}-1+\eta L\right)\left(\frac{1}{c}-1\right)+ L \left(\frac{1}{c}-1\right)^2-\frac{1}{\eta c^2}  \right]\sum_{k=0}^T\frac{\|x_k-x_{k-1}\|_2^2}{k+1}\\
    &+\frac{L}{\eta cT}\left(\frac{1}{c}-1\right)\sum_{k=0}^T\frac{\|x_k-x_{k-1}\|_2^2}{k+1}+\frac{1}{\eta^2 c T}\left(\frac{1}{c}-1\right)\sum_{k=0}^T\frac{\|x_k-x_{k-1}\|_2^2}{(k+1)^2}.
\end{split}
\end{equation}

Remark that 
\begin{align}
    \alpha_{k+1}-\alpha_k&=\frac{\sqrt{k+2}-\sqrt{k+1}}{\sqrt{k+1}}-\frac{\sqrt{k+1}-\sqrt{k}}{\sqrt{k}}\nonumber\\
    &\leq \frac{1}{2(k+1)}-\frac{1}{2\sqrt{k(k+1)}}\nonumber\\
    &=\frac{1}{2\sqrt{k+1}} \cdot  \frac{\sqrt{k}-\sqrt{k+1}}{\sqrt{k(k+1)}}  \\
    &\leq -   \frac{1}{2\sqrt{k}(k+1)^{3/2}}.
\end{align}
 
 \fi
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
 
 
 
 
 
 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sgd_proof.tex <==
\section{Convergence analysis of non-convex SGD}\label{sec:sgd_proof}

We remind the convergence analysis of non-convex SGD in the smooth setting \cite{bottou2016optimization}. 
\begin{theorem}\label{thm:sgd_rate}
Let $f$ be a smooth function. Let $x_1,\dots,x_T$ be the points returned by SGD. Set the stepsize as $\eta_k=1/\sqrt{T}$ for $k\in\{1,\dots,T\}$. Then, we have:
  \begin{equation}\label{eq:sgd_rate}
 \begin{split}
   \frac{1}{T} \sum_{t=0}^T \|\nabla f(x_t)\|^2 \leq \frac{ f(x_0)-f^*}{\sqrt{T}} +   \frac{L\sigma^2}{2T}, 
\end{split}
 \end{equation}
 where $f^*=\mathbb{E}[f(x_{T+1})]$.
\end{theorem}
\begin{proof}[Proof of \autoref{thm:sgd_rate}]
We start by applying the smoothness inequality on $f$. At a time step $k\in\{1,\dots,T\}$, we have
\begin{align}\label{eq:smoothapplyf}
    \langle \nabla f(x_k), x_k-x_{k+1}\rangle \leq f(x_t)-f(x_{t+1}) + \frac{L}{2}\|x_k-x_{k+1}\|_2^2
\end{align}
By using the SGD update \eqref{eq:update_MD} in \eqref{eq:smoothapplyf}, we obtain:
\begin{align}\label{eq:updatesmoothf}
    \eta_k\langle \nabla f(x_k),g_k\rangle \leq f(x_k)-f(x_{k+1}) + \frac{L\eta_k^2}{2}\|g_k\|_2^2.
\end{align}
Let $\mathbb{E}_k[Y]$ denote the expectation of a random variable $Y$ conditioned on $\mathcal{F}_k$, the filtration with respect to $x_0,...,x_k$.  Now, by taking the expectation conditioned on $\mathcal{F}_k$ and using the properties of the stochastic gradient oracle (\autoref{ass:sto_grad}) in \eqref{eq:updatesmoothf}, we have
\begin{align}\label{eq:expupdsmooth}
    \eta_k\|\nabla f(x_k)\|_2^2 \leq f(x_k)-\mathbb{E}_k[f(x_{k+1})] + \frac{L\eta_k^2\sigma^2}{2}.
\end{align}
Now, by summing \eqref{eq:expupdsmooth} over $k=0,\dots,T$, we obtain
\begin{align}\label{eq:sumexpupsmooth}
    \frac{1}{T}\sum_{k=0}^T\eta_k\|\nabla f(x_k)\|_2^2 \leq \frac{f(x_0)-\mathbb{E}[f(x_{T+1})]}{T} + \frac{L\sigma^2}{2T}\sum_{k=0}^T\eta_t^2.
\end{align}
By setting $f^*=\mathbb{E}[f(x_{T+1})]$ and $\eta_k=1/\sqrt{T},$ we obtain \eqref{eq:sgd_rate}.

\end{proof}
